Semantics-Preserving DPO-Based Term Graph Rewriting

Term graph rewriting is important as "conceptual implementation" of the execution of functional programs, and of data-flow optimisations in compilers. One way to define term graph transformation rule application is via the well-established and intuitively accessible double-pushout (DPO) approach; we present a new result proving semantics preservation for such DPO-based term graph rewriting.

==> eptcsdata.tex <==
\providecommand{\firstpage}{26}
\providecommand{\publicationstatus}{M. Fern\'andez and I. Mackie (Eds.): TERMGRAPH 2018.\\
EPTCS 288, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.288.3}{10.4204/EPTCS.288.3}}
\pdfoutput=1

